Rebooting ACGAN: Auxiliary Classifier GANs with Stable Training

Conditional Generative Adversarial Networks (cGAN) generate realistic images by incorporating class information into GAN. While one of the most popular cGANs is an auxiliary classifier GAN with softmax cross-entropy loss (ACGAN), it is widely known that training ACGAN is challenging as the number of classes in the dataset increases. ACGAN also tends to generate easily classifiable samples with a lack of diversity. In this paper, we introduce two cures for ACGAN. First, we identify that gradient exploding in the classifier can cause an undesirable collapse in early training, and projecting input vectors onto a unit hypersphere can resolve the problem. Second, we propose the Data-to-Data Cross-Entropy loss (D2D-CE) to exploit relational information in the class-labeled dataset. On this foundation, we propose the Rebooted Auxiliary Classifier Generative Adversarial Network (ReACGAN). The experimental results show that ReACGAN achieves state-of-the-art generation results on CIFAR10, Tiny-ImageNet, CUB200, and ImageNet datasets. We also verify that ReACGAN benefits from differentiable augmentations and that D2D-CE harmonizes with StyleGAN2 architecture. Model weights and a software package that provides implementations of representative cGANs and all experiments in our paper are available at https://github.com/POSTECH-CVLab/PyTorch-StudioGAN.

==> Paper/Figures/Figure_generated_images.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Proj_Acc.png}
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Proj_FID.png}
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Proj_SN.png}
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Contra_Acc.png}
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Contra_FID.png}
    \includegraphics[width=0.31\linewidth]{Paper/Figures/pdf/Contra_SN.png}
    \caption{Authenticity classification accuracies on the training and validation datasets (left), trends of FID values (middle), and trends of the largest singular values of the discriminator's convolutional parameters (right). To specify the starting point where the difference between the training and validation accuracies is greater than 0.5, we use a solid black line. The first and second black dotted lines indicate when the performance is best and when training collapse occurs, respectively.}
    \label{fig:Figure_generated_images}
\end{figure}

==> Paper/Figures/Figure_performance.tex <==
\begin{wrapfigure}{R}{0.53\textwidth}
  \vspace{-50pt}
  \centering
  \includegraphics[width=0.55\textwidth]{Paper/Figures/pdf/performance.pdf}
  \caption{FID improvements of DadaGAN on various datasets: \textsc{CIFAR10}~\cite{Krizhevsky2009LearningML}, \textsc{CUB200}~\cite{WelinderEtal2010}, \textsc{Tiny-ImageNet}~\cite{Tiny}, and \textsc{ImageNet}~\cite{Deng2009ImageNetAL}. The improvements are computed based on BigGAN~\cite{Brock2019LargeSG} using popular StudioGAN library~\cite{kang2020contragan}. $*$ indicates we take the FID values reported in papers~\cite{Miyato2018SpectralNF,Zhang2019SelfAttentionGA, kang2020contragan}.}
  \vspace{-8pt}
 \label{fig:Figure_performance}
\end{wrapfigure}
 

==> Paper/Figures/Figure_training_curve.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
  \vspace{-30pt}
  \centering
  \includegraphics[width=0.54\textwidth]{Paper/Figures/pdf/IS_FID_Curves.pdf}
  \vspace{3pt}
  \caption{Temporal image I will polish this CircleGAN (ours) vs. SphereGAN}
   \vspace{-10pt}
 \label{fig:Figure_training_curve}
\end{wrapfigure}
 
